QuickXsort - A Fast Sorting Scheme in Theory and Practice

QuickXsort is a highly efficient in-place sequential sorting scheme that mixes Hoare's Quicksort algorithm with X, where X can be chosen from a wider range of other known sorting algorithms, like Heapsort, Insertionsort and Mergesort. Its major advantage is that QuickXsort can be in-place even if X is not. In this work we provide general transfer theorems expressing the number of comparisons of QuickXsort in terms of the number of comparisons of X. More specifically, if pivots are chosen as medians of (not too fast) growing size samples, the average number of comparisons of QuickXsort and X differ only by $o(n)$-terms. For median-of-$k$ pivot selection for some constant $k$, the difference is a linear term whose coefficient we compute precisely. For instance, median-of-three QuickMergesort uses at most $n \lg n - 0.8358n + O(\log n)$ comparisons. Furthermore, we examine the possibility of sorting base cases with some other algorithm using even less comparisons. By doing so the average-case number of comparisons can be reduced down to $n \lg n- 1.4106n + o(n)$ for a remaining gap of only $0.0321n$ comparisons to the known lower bound (while using only $O(\log n)$ additional space and $O(n \log n)$ time overall). Implementations of these sorting strategies show that the algorithms challenge well-established library implementations like Musser's Introsort.

==> quickXsort_preamble.tex <==
% TeX root = quickXsort_journal
\newcommand{\ifdraft}[2]{\ifthenelse{\equal{\indraftmode}{true}}{#1}{#2}}

\makeatletter

%\usepackage{a4wide}
%\usepackage[noend,vlined,figure]{algorithm2e} 
\usepackage[noend,vlined]{algorithm2e} 


\usepackage{float}
\floatstyle{ruled}
\newfloat{algorithm}{tbp}{loa}
\floatname{algorithm}{Algorithm}


\usepackage{clrscode3e}
\usepackage[utf8]{inputenc}
\usepackage{ifluatex}
\ifluatex\else
\DeclareUnicodeCharacter{2212}{\ensuremath{-}}
\fi
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage{slantsc}
\AtBeginDocument{%
  \DeclareFontShape{T1}{lmr}{m}{scit}{<->ssub*lmr/m/scsl}{}%
}



\usepackage{babel}

\usepackage{array,multicol}
\usepackage{amsmath,amsfonts,amssymb,mathtools,colonequals,xfrac}
\usepackage{mleftright}\mleftright % redefine left and right to not add space around braces
\usepackage{relsize,ifthen,xspace,enumitem,booktabs,adjustbox,needspace}
\usepackage[referable]{threeparttablex}
\usepackage{graphicx}
\graphicspath{pics}

\usepackage{tikz}
\usetikzlibrary{
	arrows.meta,
	calc,
	positioning,
	patterns,
	external,
}
\usepackage{wref}
\let\prettyref\wref

\usepackage{needhspace}

\usepackage{microtype}
%\usepackage{enumerate}
\usepackage{listings}
\usepackage{multirow}


\usepackage{pgfplots}


\tikzsetexternalprefix{pics/externalized/}
\tikzexternalize[mode=list and make,up to date check=simple]

%% Use lualatex on externalized pics, avoids memory limits.
\tikzset{
	external/system call={%
		lualatex \tikzexternalcheckshellescape -halt-on-error %
			-interaction=batchmode -jobname "\image" "\texsource"%
	},
}
\tikzset{external/export=false} % Only export manually marked pictures, enable for costly pictures

\newcommand{\externalizedpicture}[1]{%
	%\tikzset{external/export=true}%
	\tikzsetnextfilename{#1}%
	\ignorespaces%
}


\usepackage{hyperref}

\makeatletter

%\usepackage[top=1.2in, bottom=1.5in, left=1.2in, right=1.2in]{geometry}
\definecolor{blue}{rgb}{0.211,0.211,0.856}
\definecolor{red}{rgb}{0.856,0.2,0.2}
%\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\blue}{\color{blue}}
\newcommand{\red}{\color{red}}

\definecolor{darkgreen}{rgb}{0.1,0.656,0.1}
\newcommand{\darkgreen}{\color{darkgreen}}

\definecolor{green}{rgb}{0.1,0.656,0.1}
\newcommand{\green}{\color{green}}

\definecolor{lgreen}{rgb}{0.411,1.0,0.411}
\definecolor{lred}{rgb}{1.0,0.711,0.501}
%\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\lgreen}{\color{lgreen}}
\newcommand{\lred}{\color{lred}}
\definecolor{lgrey}{rgb}{0.5,0.5,0.5}
\definecolor{llgrey}{rgb}{0.68,0.68,0.68}
%\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\lgrey}{\color{lgrey}}


\newenvironment{SE}{\noindent\color{red} SE : }{}
\newcommand{\see}[1]{
	\begin{SE} #1 \end{SE}}


\newenvironment{aw}{\noindent\color{green} AW :  }{}
\newcommand{\aww}[1]{
	\begin{aw} #1 \end{aw}}


\newenvironment{sw}{\noindent\color{blue} SW :  }{}
\newcommand{\sww}[1]{
	\begin{sw} #1 \end{sw}}


%%%%%%%%%%% SHORT REFS
%\newrefformat{thm}{Thm.~\ref{#1}}
%\newrefformat{lm}{Lem.~\ref{#1}}
%\newrefformat{dfn}{Def.~\ref{#1}}
%\newrefformat{cor}{Cor.~\ref{#1}} 
%\newrefformat{prop}{Prop.~\ref{#1}}
%\newrefformat{sec}{Sect.~\ref{#1}}
%\newrefformat{kap}{Chap.~\ref{#1}}
%\newrefformat{bsp}{Ex.~\ref{#1}}
%\newrefformat{eq}{(\ref{#1})}
%\newrefformat{tab}{Tab.~\ref{#1}}
%\newrefformat{fig}{Fig.~\ref{#1}}
%\newrefformat{app}{App.~\ref{#1}}

\newcommand\algorithmname[1]{\textsc{#1}\xspace}
\newcommand{\dd}{:$\!$:}
\newcommand{\stdsort}{\texttt{std:$\!$:sort}\xspace}
\newcommand{\stdpartialsort}{\texttt{std:$\!$:partial\_sort}\xspace}
\newcommand{\stdnth}{\texttt{std:$\!$:nth\_element}\xspace}
\newcommand{\stdstablesort}{\texttt{std:$\!$:stable\_sort}\xspace}



\newcommand{\QuickXsort}{\algorithmname{QuickXsort}}
\newcommand{\QuickXYsort}{\algorithmname{QuickXYsort}}
\newcommand{\CleverQuicksort}{\algorithmname{CleverQuicksort}}
\newcommand{\QuickMergeQuicksort}{\algorithmname{QuickMergeQuicksort}}
\newcommand{\QuickMergeCleverQuicksort}{\algorithmname{QuickMergeCleverQuicksort}}
\newcommand{\QuickMergeXsort}{\algorithmname{QuickMergeXsort}}
\newcommand{\QuickMergesort}{\algorithmname{QuickMergesort}}
\newcommand{\QuickHeapsort}{\algorithmname{QuickHeapsort}}
\newcommand{\Mergesort}{\algorithmname{Mergesort}}
\newcommand{\Heapsort}{\algorithmname{Heapsort}}
\newcommand{\ExternalHeapsort}{\algorithmname{ExternalHeapsort}}
\newcommand{\Quicksort}{\algorithmname{Quicksort}}
\newcommand{\Mergeinsertion}{\algorithmname{MergeInsertion}}

% number sets
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\B}{\mathbb{B}}

\newcommand{\Merge}{\mbox{$\mathit{merge}$}}

\newcommand{\Mergeinsertionrecursive}{\mbox{$\mathit{mergeinsertionrecursive}$}}
\newcommand{\Heapify}{\mbox{$\mathit{heapify}$}}
\newcommand{\Extract}{\mbox{$\mathit{extract}$}}
\newcommand{\Findmin}{\mbox{$\mathit{find}$\textnormal{-}}\allowbreak{}\mbox{$\mathit{min}$}}
\newcommand{\Insert}{\mbox{$\mathit{insert}$}}
\newcommand{\Extractmin}{\mbox{$\mathit{extract}$\textnormal{-}$\mathit{min}$}}
\newcommand{\Meld}{\mbox{$\mathit{meld}$}}
\newcommand{\Decrease}{\mbox{$\mathit{decrease}$}}
\newcommand{\Delete}{\mbox{$\mathit{delete}$}}
\newcommand{\Decreasekey}{\mbox{$\mathit{decrease}$\textnormal{-}$\mathit{key}$}}
\newcommand{\Distinguishedancestor}{\mbox{$\mathit{distinguished}$\textnormal{-}$\mathit{ancestor}$}}
\newcommand{\Repeatedinsert}{\mbox{$\mathit{repeated}${\textrm-}$\mathit{insert}$}}%
\newcommand{\Link}{\mbox{$\mathit{join}$}}
\newcommand{\Borrow}{\mbox{$\mathit{borrow}$}}
\newcommand{\Deletemin}{\mbox{$\mathit{extract}$-$\mathit{min}$}} 
\newcommand{\Bulkinsert}{\mbox{$\mathit{bulk}${\textrm-}$\mathit{insert}$}} 

\newcommand{\Construct}{\mbox{$\mathit{construct}$}}
\newcommand{\Binaryinsert}{\mbox{$\mathit{binary}${\textrm-}$\mathit{insert}$}}
\newcommand{\Dualconstruct}{\mbox{$\mathit{dual}${\textrm-}$\mathit{construct}$}}
\newcommand{\Dancestor}{\mbox{$\mathit{d}$\mbox{\textrm-}$\mathit{ancestor}$}}
\newcommand{\Dchild}{\mbox{$\mathit{d}$\mbox{\textrm-}$\mathit{child}$}}
\newcommand{\Siftdown}{\mbox{$\mathit{sift}$\mbox{\textrm-}$\mathit{down}$}}
\newcommand{\Siftup}{\mbox{$\mathit{sift}$\mbox{\textrm-}$\mathit{up}$}}
\newcommand{\DfConstruct}{\mbox{$\mathit{df}$\mbox{\textrm-}$\mathit{construct}$}} 

\newcommand{\Oh}{\mathcal{O}}
\newcommand{\oh}{o} 
\newcommand{\abs}[1]{\left|\mathinner{#1}\right|}
\newcommand{\Abs}[1]{\left\Vert\mathinner{#1}\right\Vert}
\newcommand{\floor}[1]{\left\lfloor\mathinner{#1} \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil\mathinner{#1} \right\rceil}
\newcommand{\set}[2]{\left\{\, \mathinner{#1}\vphantom{#2}\: \left|\: \vphantom{#1}\mathinner{#2} \right.\,\right\}}

%%%%%%%% Probas
%\renewcommand{\Pr}[1]{\mathop{\mathrm{Pr}}\left[\,#1\,\right]}
\providecommand{\DontPrintSemicolon}{\dontprintsemicolon}



%% Thm-like environments
\usepackage[amsmath,hyperref,thmmarks]{ntheorem}

\theoremseparator{:}
\theoremstyle{plain}
\theorembodyfont{\slshape}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
%
%\theoremstyle{break}
%\newtheorem{lemmabr}[theorem]{Lemma}
%\theoremstyle{plain}
%\theorembodyfont{\upshape}
%\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}


\theorembodyfont{\upshape}
\newtheoremstyle{proofstyle}%
{\item[\theorem@headerfont\hskip\labelsep ##1\theorem@separator]}%
{\item[\theorem@headerfont\hskip\labelsep ##1 of ##3\theorem@separator]}
\theoremstyle{proofstyle}
\theoremsymbol{\raisebox{-.25ex}{$\Box$}}
\qedsymbol{\raisebox{-.25ex}{$\Box$}}

\newtheorem{proof}{Proof}

\newenvironment{thmenumerate}[1]{%
	\begin{enumerate}[
		label={\makebox[\widthof{(a)}][c]{\textup{(\alph*)}}},
		ref={\ref{#1}\kern.1em--\kern.1em(\alph*)},
		itemsep=0pt,
	]%
}{%
	\end{enumerate}%
}






% page style setup
\setlength\parindent{1.5em}
\usepackage{colonequals}
%	
\usepackage[headsepline]{scrlayer-scrpage}
\pagestyle{scrheadings}
\clearscrheadfoot
\AtBeginDocument{%
	\manualmark%
	\markleft{\mytitle}%
	\automark*[section]{}%
}
\ohead{\pagemark}
\ihead{\headmark}
%	
\addtokomafont{caption}{\sffamily\small}
\addtokomafont{captionlabel}{\sffamily\textbf}
\setcapmargin{2em}










% Box hacks

%%%%% create an hbox of the given width height and depth
%%%%% beware, ugly TeX hack, may result in strange
%%%%% behavior
\def\makeboxwhd#1#2#3#4{\setbox0=\hbox{#4}%
\ht0=#2%
\dp0=#3%
\wd0=#1%
\box0%
}

\newcommand*{\vcenteredhbox}[1]{\begingroup
\setbox0=\hbox{#1}\parbox{\wd0}{\box0}\endgroup}


%%%%% create an hbox of the size of #2, but insert #3
%%%%% #1 can be l, c or r and gives the horizontal position
\newdimen\makeboxdimen
%\setlength\fboxsep{-\fboxrule}
\newcommand\makeboxlike[3][l]{%
\setbox0=\hbox{#2}%
\global\makeboxdimen=\wd0%
\setbox1=\hbox{\makebox[\makeboxdimen][#1]{%
\makebox[0pt][#1]{#3}%
}}%
\ht1=\ht0%
\dp1=\dp0%
\box1%	
}


\newcommand\plaincenter[1]{%
	\ignorespaces%
		\mbox{}\hfill#1\hfill\mbox{}
	\unskip%
}

% Common phrases
\newcommand*\ie{\mbox{i.\hspace{.2ex}e.}}
\newcommand*\eg{\mbox{e.\hspace{.2ex}g.}}
\newcommand*\iid{\mbox{i.\hspace{.2ex}i.\hspace{.2ex}d.}\xspace}
\newcommand*\wrt{\mbox{w.\hspace{.2ex}r.\hspace{.2ex}t.}\xspace}
\newcommand*\aka{\mbox{a.\hspace{.2ex}k.\hspace{.2ex}a.}\xspace}
\newcommand*\withoutlossofgenerality{\mbox{w.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\Withoutlossofgenerality{\mbox{W.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\almostsurely{\mbox{a.\hspace{.2ex}s.}\xspace}
\newcommand*\whp{\mbox{w.\hspace{.2ex}h.\hspace{.2ex}p.}\xspace}


	
%%%%% OFTEN USED MATH MACROS
\newcommand{\ESymbol}{\mathbb{E}}
\newcommand\Eop{%
	\mathop{\mathchoice{%display
		\text{$\ESymbol$}%
	}{%text
		\text{$\ESymbol$}%
	}{%script
		\text{\scriptsize$\ESymbol$}%
	}{%scriptscript
		\text{\tiny$\ESymbol$}%
	}%
	}\nolimits%
}
\def\.{\mskip1mu} 

%\newcommand*\llbracket{\mathopen{[\mkern-2.5mu[}}
%\newcommand*\rrbracket{\mathclose{]\mkern-2.5mu]}}

\newcommand\leftatop[2]{\genfrac{}{}{0pt}{}{#1\hfill}{#2\hfill}}

\newcommand{\openball}[2][\varepsilon]{\mathrm B_{<{#1}}\left(#2\right)}
\newcommand{\closedball}[2][\varepsilon]{\mathrm B_{\le{#1}}\left(#2\right)}

\DeclareMathOperator\ld{ld}
\DeclareMathOperator\hd{hd}

\newcommand{\VarSymbol}{\ensuremath{\mathrm{Var}}}
\newcommand{\CovSymbol}{\ensuremath{\mathrm{Cov}}}
\newcommand{\ProbSymbol}{\ensuremath{\mathbb{P}}}
\providecommand{\given}{}
%% mathtools command to declare cool delimiter pairs:
%	\DeclarePairedDelimiterXPP{cmd}[numargs]{pre code}{left_delim}{right_delim}{post code}{body}
\DeclarePairedDelimiterXPP\Prob[1]{\ProbSymbol}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#1%
}
\DeclarePairedDelimiterXPP\E[1]{\ESymbol}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#1%
}
\DeclarePairedDelimiterXPP\Eover[2]{\ESymbol_{#1}}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#2%
}
\DeclarePairedDelimiterXPP\Var[1]{\VarSymbol}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#1%
}
\DeclarePairedDelimiterXPP\Cov[1]{\CovSymbol}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#1%
}
\providecommand{\Prob}{} % hack for syntax highlighting ...
\providecommand{\E}{} % hack for syntax highlighting ...
\providecommand{\Eover}{} % hack for syntax highlighting ...
\providecommand{\Var}{} % hack for syntax highlighting ...
\providecommand{\Cov}{} % hack for syntax highlighting ...


\newcommand\disjointunion{\mathbin{\dot{\cup}}}

\newcommand\total[1]{\Sigma #1}
\newcommand\product[1]{\Pi #1}

\newcommand\ui[2]{#1^{\smash{(}#2\smash{)}}}
% Upper index macro (Algorithmica math style uses too large parentheses for simply writing x^{(1)}.
% \newcommand{\ui}[2]{%
% 	\mathchoice{%display
% 		%#1^{\smash{(}#2\smash{)}}%
% 		#1^{(#2)}%
% 	}{%text
% 		#1^{%
% 			\smash{\raisebox{.75pt}{\mbox{\tiny$($}}}%
% 			#2%
% 			\smash{\raisebox{.75pt}{\mbox{\tiny$)$}}}%
% 		}%
% 	}{%script
% 		#1^{\smash{(}\rule[-.75pt]{0pt}{2.75pt}#2\smash{)}}%
% 	}{%scriptscript
% 		#1^{(#2)}%
% 	}%
% }

\usepackage{fixmath}
\newcommand{\vect}[1]{\boldsymbol{\mathbold{#1}}}
%\newcommand{\vect}[1]{\boldsymbol{\mathbf{#1}}}

\newcommand\eqdist{	
	\mathchoice{%display
		\mathrel{\overset{\raisebox{0ex}{$\scriptstyle \mathcal D$}}=}%
	}{%text
		\mathrel{\like{=}{%
			\overset{\raisebox{-1ex}{$\scriptscriptstyle \mathcal D$}}=%
		}}%
	}{%script
		\mathrel{\overset{\mathcal D}=}%
	}{%scriptscript
		\mathrel{\overset{\mathcal D}=}%
	}%
}
\newcommand\eqdistt{\mathrel{\smash{\stackrel{\scriptscriptstyle\mathcal D}=}}}
\let\eqlaw\eqdist

\newcommand*\lest{\mathrel{\le_{\mathrm{st}}}}

\newcommand\pe{\phantom{{}={}}}
\newcommand\ppe{\phantom{=}}

\newcommand\like[3][c]{%
	\mathchoice{%dis
		\makeboxlike[#1]{%
			\ensuremath{\displaystyle\relax#2}%
		}{%
			\ensuremath{\displaystyle\relax#3}%
		}%
	}{%txt
		\makeboxlike[#1]{%
			\ensuremath{\textstyle\relax#2}%
		}{%
			\ensuremath{\textstyle\relax#3}%
		}%
	}{%sc
		\makeboxlike[#1]{%
			\ensuremath{\scriptstyle\relax#2}%
		}{%
			\ensuremath{\scriptstyle\relax#3}%
		}%
	}{%scsc
		\makeboxlike[#1]{%
			\ensuremath{\scriptscriptstyle\relax#2}%
		}{%
			\ensuremath{\scriptscriptstyle\relax#3}%
		}%
	}
}


\newcommand\uniform{\mathcal U}
\newcommand{\exponentialDist}{\mathrm{Exp}}
\newcommand\normaldist{\mathcal N}
\newcommand\bernoulli{\mathrm B}
\newcommand\hypergeometric{\mathrm{HypG}}
\newcommand\multinomial{\mathrm{Mult}}
\newcommand\binomial{\mathrm{Bin}}
\newcommand\dirichlet{\mathrm{Dir}}
\newcommand\betadist{\mathrm{Beta}}
\newcommand\gammadist{\mathrm{Gamma}}
\newcommand\betaBinomial{\mathrm{BetaBin}}
\newcommand\dirichletMultinomial{\mathrm{DirMult}}
\newcommand\poissondist{\mathrm{Pois}}


\DeclarePairedDelimiterXPP\distFromWeights[1]{\mathcal D}(){}{#1}
\providecommand\distFromWeights{} %hack for syntax highlighting

\newcommand\BetaFun{\mathrm B}
\newcommand{\polylog}[2][\alpha]{\mathrm{Li}_{#1}\left(#2\right)}

\renewcommand\given{\mathbin{\mid}}
% Harmonic Numbers
\newcommand\harm[1]{\ensuremath{H_{#1}}}


\newcommand\Aint{\smallint\nolimits_A}
\newcommand\Bint{\smallint\nolimits_B}



\newcommand\ce{\colonequals}

\newcommand{\surroundedmath}[3]{% #1=mathrel/mathbin/etc #2=spacing #3=symbol
	\mathchoice{%display
		#1{#2{#3}#2}%
	}{%text
		#1{#3}%
	}{%script
		#1{#3}%
	}{%scriptsript
		#1{#3}%
	}%
}

\newcommand\rel[1]{\surroundedmath{\mathrel}{\:}{#1}}
\newcommand\wrel[1]{\surroundedmath{\mathrel}{\;}{#1}}
\newcommand\wwrel[1]{\surroundedmath{\mathrel}{\;\;}{#1}}
\newcommand\bin[1]{\surroundedmath{\mathbin}{\:}{#1}}
\newcommand\wbin[1]{\surroundedmath{\mathbin}{\;}{#1}}
\newcommand\wwbin[1]{\surroundedmath{\mathbin}{\;\;}{#1}}

\newcommand{\eqwithref}[2][c]{%
	\relwithref[#1]{#2}{=}%
}
\newcommand{\relwithref}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize\wref{#2}}}}{#3}}%
}
\newcommand{\relwithtext}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize#2}}}{#3}}%
}


% Make align suppress number for \\* lines
% define galign to use subequation labels
\makeatletter
\let\oldalign\align
\let\endoldalign\endalign

\newcommand*\numberthis[1][]{\stepcounter{equation}\tag{\theequation}}

\renewenvironment{align}{%
	\begingroup%
	\let\oldhalign\halign
	\def\halign{%
		\let\oldbreak\\%
		\def\nonnumberbreak{\nonumber\oldbreak*}%
		\def\\{%
			\@ifstar{\nonnumberbreak}{\oldbreak}%
		}%
		\oldhalign%
	}
	\let\oldlabel\label%
	\oldalign%
}{%
	\endoldalign%
	\endgroup%
}

\newenvironment{galign}[1][]{%
	\subequations%
	#1%
%	\def\theequation{\theparentequation--\alph{equation}}%
	\def\theequation{\theparentequation{\protect\footnotesize\hspace{.1em}.\arabic{equation}}}%
%	\def\theequation{\theparentequation\rlap{~\,--\,\alph{equation}}}%
	\align%
}{%
	\endalign%
	\endsubequations%
}


\newcommand\tagref[2][\width]{%
	\tag*{\makebox[#1][r]{\wref{#2} \scriptsize revisited}}%
}


\newcommand\separatedpar{%
	\medskip
	\plaincenter{%
		$*$\hspace{3em}$*$\hspace{3em}$*$%
	}\par
	\medskip
	\noindent
}


% Notation list
\def\mydots{\xleaders\hbox to.5em{\hfill.\hfill}\hfill}


\newlength\tmpLenNotations
\newenvironment{notations}[1][10em]{%
	\small
	\newcommand\notationentry[1]{%
		\settowidth\tmpLenNotations{##1}%
		\ifthenelse{\lengthtest{\tmpLenNotations > \labelwidth}}{%
			\parbox[b]{\labelwidth}{%
				\makebox[0pt][l]{##1}\\%
			}%
		}{%
			\mbox{##1}%
		}%
		\mydots\relax%
	}%
	\begin{list}{}{%
		\setlength\labelsep{0em}%
		\setlength\labelwidth{#1}%
		\setlength\leftmargin{\labelwidth+\labelsep+1em}%
		\renewcommand\makelabel{\notationentry}%
	}
	\newcommand\notation[1]{\item[{##1}]}%
	\raggedright
}{%
	\end{list}
}
\newcommand*\phdthesis{\mbox{Ph.\hspace{.2ex}D.} thesis\xspace}




%%%%% Allow page breaks in display math environments 
%%%%% With this, display environments can be broken as paragraphs.
%%%%% The 1 means that such breaks should be considered not nice, but acceptable.
\allowdisplaybreaks[3]


% Alter some LaTeX defaults for better treatment of figures:
    % See p.105 of "TeX Unbound" for suggested values.
    % See pp. 199-200 of Lamport's "LaTeX" book for details.
    %   General parameters, for ALL pages:
    \renewcommand{\topfraction}{0.9}	% max fraction of floats at top
    \renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom
    %   Parameters for TEXT pages (not float pages):
    \setcounter{topnumber}{2}
    \setcounter{bottomnumber}{2}
    \setcounter{totalnumber}{4}     % 2 may work better
    \setcounter{dbltopnumber}{2}    % for 2-column pages
    \renewcommand{\dbltopfraction}{0.9}	% fit big float above 2-col. text
    \renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
    %   Parameters for FLOAT pages (not text pages):
    \renewcommand{\floatpagefraction}{0.8}	% require fuller float pages
% N.B.: floatpagefraction MUST be less than topfraction !!
    \renewcommand{\dblfloatpagefraction}{0.8}	% require fuller float pages



\let\oldthebibliography\thebibliography
\renewcommand\thebibliography[1]{%
	\oldthebibliography{#1}%
	\pdfbookmark[1]{References}{}%
	\markleft{\mytitle} % overwrite refs mark
}


\let\epsilon\varepsilon
% Put a dot behind title of paragraph
\let\oldparagraph\paragraph
\renewcommand\paragraph{%
    \@ifstar{\myparagraphStar}{\myparagraphNoStar}%
}
\newcommand\myparagraphStar[1]{%
	\oldparagraph*{#1.}%
}
\newcommand\myparagraphNoStar[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\oldparagraph[#2]{#2.}%
	}{%
		\oldparagraph[#1]{#2.}%
	}%
}




\RequirePackage[textsize=tiny,textwidth=2.4cm,
	%backgroundcolor=orange!20,
	backgroundcolor=white,
	bordercolor=red!80!black,
	shadow]{todonotes} 

\newcommand\todoin[2][]{%
	\todo[inline, caption={2do}, bordercolor=red!80!black, size=\footnotesize, #1]{%
	\begin{minipage}{\linewidth-1em}%
		\setlength{\parskip}{1ex}%
		\noindent\relax\ignorespaces#2\ignorespaces%
	\end{minipage}}%
}

\ifdraft{%
	% Show overfull boxes (without activating draft mode)
	\overfullrule=6mm
	
	%%%% Hacks to show labels, ref and cite keys
	\usepackage[color,notref,notcite]{showkeys}
	\definecolor{refkey}{gray}{.99}
	\colorlet{labelkey}{green!60!black!60}
	\renewcommand{\showkeyslabelformat}[1]{%
	  \adjustbox{scale={.9}{.9}}{\scriptsize{\texttt{#1}}}%
	}
	\usepackage[inline,nolabel]{showlabels}
	\renewcommand{\showlabelsetlabel}[1]{%
	  \adjustbox{scale={.8}{.9}}{\textcolor{blue!50!black!45}{\scriptsize{\texttt{#1}}}}%
	}
	\renewcommand\showlabelrefline{%
		\color{blue!55!black!35}\hrule width 0pt height 1.5ex depth 0pt%
	}
	\showlabels{cite}
	\showlabels{citealt}
	\showlabels{citealp}
	\showlabels{citet}
	\showlabels{Citet}
	\showlabels{citep}
	\showlabels{citeauthor}
	\showlabels{Citeauthor}
	\showlabels{citefullauthor}
	\showlabels{citeyear}
	\showlabels{citeyearpar}
	\showlabels{wref}
	\showlabels{wpref}
	\showlabels{wtpref}
	\showlabels{wildref}
	\showlabels{wildpageref}
	\showlabels{wildtpageref}
}{}

\ifdraft{}{%
	\usepackage{microtype}
}

